An Achilles' Heel of Term-Resolution

Term-resolution provides an elegant mechanism to prove that a quantified Boolean formula (QBF) is true. It is a dual to Q-resolution (also referred to as clause-resolution) and is practically highly important as it enables certifying answers of DPLL-based QBF solvers. While term-resolution and Q-resolution are very similar, they're not completely symmetric. In particular, Q-resolution operates on clauses and term-resolution operates on models of the matrix. This paper investigates what impact this asymmetry has. We'll see that there is a large class of formulas (formulas with "big models") whose term-resolution proofs are exponential. As a possible remedy, the paper suggests to prove true QBFs by refuting their negation ({\em negate-refute}), rather than proving them by term-resolution. The paper shows that from the theoretical perspective this is indeed a favorable approach. In particular, negation-refutation can p-simulates term-resolution and there is an exponential separation between the two calculi. These observations further our understanding of proof systems for QBFs and provide a strong theoretical underpinning for the effort towards non-CNF QBF solvers.

==> bl.tex <==
% File:  bl.tex
% Author: mikolas
% Created on: Sun, Apr 21, 2013 7:16:13 PM
% Copyright (C) 2013, Mikolas Janota
\section{Blocked Clause}
The formula \autoref{equation:iff} enables us to show a separation
between term-resolution and negation-refutation. However, this
formula has another interesting property and that is that it can be
completely solved by the blocked clause elimination technique, commonly
used in preprocessing~\cite{BiereEtAlCADE11}.

\begin{definition}[blocked clause~\cite{BiereEtAlCADE11}]
For a  QBF $P.\ \phi$,  and a clause $C\in\phi$  a literal $l\in C$  is {\em blocked} iff
 for any cause $C'\in\phi$ s.t.\ $\bar l\in C'$  there is a literal $k$ with 
$\lev(k)\leq\lev(l)$, $k\in C'$, and $\bar k\in C'$.
%
 A clause is a {\em blocked clause} iff  it contains at least one blocked literal.
\end{definition}

\paragraph{Note.} A more advanced definition can be found in~\cite{DBLP:conf/sat/GelderWL12}.

Let $x$ be a blocked literal in a clause $B$.
Further, consider the set of clauses $C_1,\ldots,C_m$ 
of those in only those clauses that contain the literal $\bar x$. From the definition of a black literal, for each of $C_i$ there is a literal $ k_i $, such that
$k_i\in B$,
$\bar k_i\in C_i$, and $\level(k_i)\leq\level(x) $.



==> blocked_clauses.tex <==
% File:  blocked_clauses.tex
% Author: mikolas
% Created on: Tue, Apr 09, 2013 5:16:19 PM
% Copyright (C) 2013, Mikolas Janota
In this section we show that if blocked clauses are used as a
preprocessing step, term resolution proofs cannot be polynomially
reconstructed.  More precisely, we construct an infinite sequence of
formulas $\Psi_1,\dots$ s.t.\ $\Psi_i$ can be preprocessed into
$\Psi_i'$ by polynomial number of blocked clause eliminations, and,
any term resolution proof of $\Psi_i$ is exponential in the size of
$\Psi_i$ while, $\Psi_i'$ can be proven in a constant number of
steps.\todo{This could be phrased in terms of a proof system that uses
  blocked clause elimination as a rule.}


 \begin{proposition}
   All clauses are blocked in~\eqref{equation:iff}, giving the empty
   CNF in a linear number of blocked clause eliminations.
 \end{proposition}

\subsection {Blocked Clause}

\begin{definition}[blocked clause~\cite{BiereEtAlCADE11}]
For a  QBF $P.\ \phi$,  and a clause $C\in\phi$  a literal $l\in C$  is {\em blocked} iff
 for any cause $C'\in\phi$ s.t.\ $\bar l\in C'$  there is a literal $k$ with 
$\lev(k)\leq\lev(l)$, $k\in C'$, and $\bar k\in C'$.
%
 A clause is a {\em blocked clause} iff  it contains at least one blocked literal.
\end{definition}

\paragraph{Note.} A more advanced definition can be found in~\cite{DBLP:conf/sat/GelderWL12}.

